Phasor-Pursuit Directional Modulation

Emitting phased array RF systems have to contend with an ever-increasing number of eavesdroppers as technological advancements provide lower cost and/or more capable radios. Often, eavesdroppers can accumulate sufficient information transmitted in sidelobes by integrating over long enough periods. Directional modulation (DM) disrupts this capability by inducing a randomized walk through IQ-space to reach a pertinent location which corresponds to a symbol of particular amplitude and phase. This results in higher secrecy capacity. The path taken by the cumulative element contributions are determined by the complex weights of individual transmitters. Because large phased arrays support a large number of available paths, repetitions of applied weights are not concerning. The same cannot be said for arrays that consist of only a few elements, e.g. WiFi routers. We introduce a computationally efficient and flexible framework for DM that utilizes real-valued phase rotations of element weights. It supports a wide family of modulation schemes in phase and/or amplitude. Using state-of-the-practice orthogonal noise injection framework, we demonstrate a richness of unique paths resolving concerns about repeated weights. In our proposed scheme, there is a small reduction in received power compared to traditional beamforming, as little as 1 dB, which is an advantage over conventional directional modulation which typically sacrifices 6 dB of power. Also, there is a significantly larger set of possible element weights than that of the conventional scheme. This feature protects against the possibility of eavesdroppers breaking the distortion-based obfuscation of symbols over repeated observations. Our approach provides more secrecy capacity than conventional directional modulation via increased power delivery and increased receiver SNR and does so with resilience to advanced eavesdropping threats.

==> background.tex <==
\begin{section}{Background}\label{section2}
Herein we present the salient mathematical features of DM to aid in denoting the differing, noteworthy, behaviors between conventional and real-valued phase approaches to DM. This discussion is concluded with the operational scenario that is used as the exemplar, and corresponding conventional DM performance, which will be used as the operational scenario for future discussions on the performance benefits and differences between conventional and real-valued phase DM unless specified otherwise.

\subsection{Mathematical Description}
We assume isotropically-radiating antenna elements with uniform array spacing of one half wavelength. The far-field pattern, $\mathbf{E}(\theta)$, is determined as a sum of the individual element contributions with the respective element excitations $\alpha_n$,
\begin{equation}\label{ff}
  \mathbf{E}(\theta)=\sum_{n=1}^N(\alpha_n e^{i\pi(n-\frac{N+1}{2})cos(\theta)}).
\end{equation}
Implementing DM is achieved through replacing the individual element excitations with the product of the modulated data stream (at symbol level) and complex gain; the gain of which possesses unity magnitude and non-zero phase in the IQ-space, i.e. $\alpha_n \equiv d_m G^*_{n}$ and $G_{n} = e^{j\phi_n}$.
\par
Moving from a single epoch to multiple epoch processing of DM sequences introduces the requirement of constraining orthogonality across the gain \textit{differences} over the array. Consider two epochs, wherein the gain coefficients can be represented via vectors $\vec{G}_u$ and $\vec{G}_v$ respectively. The gain difference is simply, $\Delta \vec{G}=\vec{G}_u-\vec{G}_v$. Then, discretizing over the spatial direction in Eq.~\ref{ff}, we denote the discrete channel matrix as
\begin{equation}\label{ch}
 \mathbf{H}\equiv
 \begin{bmatrix}
  e^{i(1-\frac{N+1}{2})\pi cos(\theta_1)} & \hdots & e^{i(N-\frac{N+1}{2})\pi cos(\theta_1)} \\
  e^{i(1-\frac{N+1}{2})\pi cos(\theta_2)} & \hdots & e^{i(N-\frac{N+1}{2})\pi cos(\theta_2)} \\
  \vdots & \ddots & \vdots \\
  e^{i(1-\frac{N+1}{2})\pi cos(\theta_K)} & \hdots & e^{i(N-\frac{N+1}{2})\pi cos(\theta_K)}
 \end{bmatrix}.
\end{equation}
We then can denote the orthogonality constraint, as presented in \cite{DingFusco2}, as
\begin{equation}
 \mathbf{H}(\theta_k = \theta_{target})^*\Delta\vec{G} = 0~.
\end{equation}

\par
We can now note the primary difference between conventional and real-valued phase DM. Conventional DM systems, such as those defined in \cite{DingFusco1,DalyBernhard2} constrain the phase of the complex gain coefficient to three values $\phi_n = [-\pi/2, 0, \pi/2]$. Whereas in the real-valued phase DM framework, we denote $\phi_n$ as a random variable drawn from a beta distribution in the interval $\phi_n \in [-\pi/2, \pi/2]$, that is $\phi_n \sim \frac{\pi}{2}[\Be(\alpha=\beta)-.5]$. We present the coefficient determination algorithm in Algorithm~\ref{alg:alg1}.\par
The implications of our modifications to the DM framework are more readily assessed in the framework of vector synthesis presented in \cite{DingFusco2,DingFusco2014}. Wherein we examine the received symbol as a superposition of vector contributions from the individual emitters in IQ space; see Fig.~\ref{superpos} where we present a simple case of conventional DM with an eight element ULA.
\begin{figure}[h!]
 \centering
 \includegraphics[width=9cm,height=4cm,keepaspectratio]{figs/vecpi2.png}
 \caption{Illustrative example of a vector path obtained through an array excitation approach consistent with conventional DM}
 \label{superpos}
\end{figure}
\begin{figure}[h!]
 \centering
 \includegraphics[width=9cm,height=4cm,keepaspectratio]{figs/vecreal.png}
 \caption{Vector path in IQ-space obtained through the real-valued phase DM approach.}
 \label{superpos2}
\end{figure}\\
Here we observe that two of the eight emitters performed a $\pm\pi/2$ rotation resulting in an approximate 2.5 dB loss. It is an easy exercise to note the difficulty in finding unique paths through IQ space which are induced by the cumulation of orthogonal array contributions when the array has relatively few elements. Within this problem space, we can easily denote the benefit of the real-valued phase framework for DM. In Fig.~\ref{superpos2} we demonstrate the effect that the real-valued phase rotations has on the vector path in IQ-space. It is important to note the behavior of two vector contributions, where an optimized close-out procedure is performed to reach the appropriate symbol phase and amplitude. This result is achieved through assessing the geometry of the vector path and constructing and appropriate equilateral triangle with the final element contributions, before a final scrambling operation distributes the phases across the array.

\subsection{Permutation}
\begin{figure}[h!]
 \centering
 \includegraphics[width=9cm,height=4cm,keepaspectratio]{figs/permute.png}
 \caption{Vector path of permuted gain sequences in the real-valued phase approach to DM.}
 \label{permute}
\end{figure}
As we have alluded to, the motivation for including real-valued phase rotations in the coefficient determination for DM beamforming was to increase the configuration diversity. This decreases the periodicity of repetition in DM transmissions which decreases the likelihood of collecting enough information by eavesdroppers to intercept the transmission and effectively decode the DM. In the limit of large, dense, phased arrays it may become too cumbersome to repeatedly compute the individual phase rotations at the symbol rate. In this situation it is important to note that permutations and reflections about the symbol axis in IQ-space can be performed for low-cost determination of additional sequences of gain coefficients across the array. As an example, consider the case presented in Fig.~\ref{permute} which shows a permuted case of vector paths for DM utilizing the real-valued phase framework in our exemplar presented herein.

\begin{figure*}[hb!]
 \centering
 \includegraphics[width= 8cm,height=8cm,keepaspectratio]{figs/taveConvDM.png}
 \includegraphics[width= 8cm,height=8cm,keepaspectratio]{figs/varConvDM.png}
 \caption{Time average (left) and variance (right) of radiation pattern for a 16 element ULA performing conventional DM over 200 epochs.}
 \label{convDMRad}
\end{figure*}
\begin{figure*}[h!]
\centering
\includegraphics[width= 16cm,height=8cm,keepaspectratio]{figs/compositephaseConvDM.png}
\caption{Phase deviation in vertical transect through target location showing the mean and min/max deviation from the average.}
\label{phaseConv}
\end{figure*}
\subsection{Exemplar}
For ease of analysis we consider a linear phased uniform line array (ULA) with operational frequency of 1 GHz. The phased array consists of $N=16$ elements separated by the conventional $\lambda/2$ spacing. Each element is capable of transmitting with maximum, unity, gain and is steering the main lobe response at $0^\circ$ from the array normal. We define eavesdroppers as receiving platforms located at angular positions outside of the main lobe response. The scenario embodies a dynamic scene with stationary transmitter and receiver platform(s), i.e. symbol rate differences are implied in the transmit scheme. Within each epoch the DM framework must match a symbol corresponding to $0^\circ$ phase and amplitude $75\%$ of total array power, that is an approximate 2.5 dB loss in intended recipient direction when compared to conventional beamforming techniques.

\subsection{Conventional DM}

We apply conventional DM to the exemplar presented above and examine the performance of the transmitting platform over a time-varying scenario. This allows us to examine the variability that the DM paradigm is capable of introducing in the radiation placed off-target. This is most readily observed in the variance and average of the radiation pattern over several epochs, each epoch presenting with the generation of a new set of phase rotations.


We present the results for conventional DM in Fig.~\ref{convDMRad} over an operational period comprising 200 independent transmission epochs. The results demonstrate the ability of the conventional DM framework to disrupt eavesdropper interception capability by causing the received energy to be unreliable over time. This effect is limited to directions that do not correspond to the intended direction. As we would expect, the variance vanishes as we approach the intended transmission direction which is a consequence of the orthogonality constraint and implying no, or limited, impact for the intentional link.
\par
The results contained in Fig.~\ref{convDMRad} are bolstered by the ability of conventional DM to provide epoch-to-epoch scrambling of phase for the symbol location in the constellation. We provide this for conventional DM in Fig.~\ref{phaseConv} where we observe a full $\pi$ of symbol phase variability at solid angles of approximately $11^\circ$.


\end{section}

